Vector-boson pair production and electroweak corrections in HERWIG++

The detailed study of vector-boson pair production processes at the LHC will lead to a better understanding of electroweak physics. As pointed out before, a consistent inclusion of higher-order electroweak effects in the analysis of corresponding experimental data may be crucial to properly predict the relevant phenomenological features of these important reactions. Those contributions lead to dramatic distortions of invariant-mass and angular distributions at high energies, but may also significantly affect the cross section near threshold, as is the case e.g. for Z-pairs. For this reason, we present an analysis of the next-to-leading-order electroweak corrections to WW, WZ and ZZ production at the LHC, taking into account mass effects as well as leptonic decays. Hence, our predictions are valid in the whole kinematic reach of the LHC and, moreover, respect the spin correlations of the leptonic decay products at NLO accuracy. Starting from these fixed-order results, a simple and straight-forward method is motivated to combine the electroweak corrections with state-of-the-art Monte Carlo predictions, focusing on a meaningful combination of higher-order electroweak and QCD effects. To illustrate our approach, the electroweak corrections are implemented in the HERWIG++ generator, and their phenomenological effects within a QCD environment are studied explicitly.

==> setup.tex <==
%\usepackage{graphics}
\usepackage{amsmath}
\usepackage{slashed}
\usepackage{cite}
%\usepackage{axodraw}
\usepackage{rotating}
\usepackage{url}
%\usepackage{feynarts}

\hfuzz .5pt

\makeatletter
 \setlength{\clubpenalty}{10000}
 \setlength{\widowpenalty}{10000}
 \setlength{\displaywidowpenalty}{10000}

\arraycolsep 2pt
\footnotesep 14pt

\if@twoside \oddsidemargin -17pt \evensidemargin 00pt
\else \oddsidemargin 00pt \evensidemargin 00pt
\fi
\topmargin 00pt \headheight 00pt \headsep 00pt
%\footheight 12pt \footskip 30pt
\textheight 230mm \textwidth 161mm

%\def\section{\@startsection {section}{1}{\z@}{+3.0ex plus +1ex minus
% +.2ex}{2.3ex plus .2ex}{\normalsize\bf}}
%\def\subsection{\@startsection{subsection}{2}{\z@}{+2.5ex plus +1ex
%minus +.2ex}{1.5ex plus .2ex}{\normalsize\bf}}
%\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{+3.25ex plus
% +1ex minus +.2ex}{1.5ex plus .2ex}{\normalsize\bf}}

\expandafter\ifx\csname mathrm\endcsname\relax\def\mathrm#1{{\rm #1}}\fi

% Equation Numbering
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\newcounter{saveeqn}
\newcommand{\alpheqn}{\setcounter{saveeqn}{\value{equation}}%
   \addtocounter{saveeqn}{1} \setcounter{equation}{0}%
   \renewcommand{\theequation}%
   {{\thesection.\arabic{saveeqn}\alph{equation}}}}
\newcommand{\reseteqn}{\setcounter{equation}{\value{saveeqn}}%
   \renewcommand{\theequation}{\thesection.\arabic{equation}}}
 
\@addtoreset{equation}{section}

\makeatother

\renewcommand{\topfraction}{0.7}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.3}
\renewcommand{\floatpagefraction}{0.7}

%\allowdisplaybreaks[3]

% new commands
\def\REF#1#2{\\[-4cm] \hspace*{#1} \rlap{\vphantom{\rule{1mm}{4cm}}
        \parbox[b]{16cm}{\baselineskip 16pt{\normalsize #2}}}}
\def\co{\relax}
\def\co{,}
\def\nl{\nonumber\\}
\def\nlc{\co\nonumber\\}
\def\nln{\nonumber\\*[-1ex]\phantom{\fbox{\rule{0em}{2ex}}}}
\def\eqskipcorr{\vspace{-\abovedisplayskip}
                \vspace{\abovedisplayshortskip}}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqar{\begin{eqnarray}}
\def\eeqar{\end{eqnarray}}
\def\barr#1{\begin{array}{#1}}
\def\earr{\end{array}}
\def\bfi{\begin{figure}}
\def\efi{\end{figure}}
\def\btab{\begin{table}}
\def\etab{\end{table}}
\def\bce{\begin{center}}
\def\ece{\end{center}}
\def\nn{\nonumber}
\def\disp{\displaystyle}
\def\text{\textstyle}
\def\arraystretch{1.4}


% shorthands for greek letters
\def\al{\alpha}
\def\be{\beta}
\def\ga{\gamma}
\def\de{\delta}
\def\veps{\varepsilon}
\def\la{\lambda}
\def\si{\sigma}
\def\Ga{\Gamma}
\def\De{\Delta}
\def\La{\Lambda}

% new commands for cross referencing
\def\refeq#1{\mbox{(\ref{#1})}}
\def\reffi#1{\mbox{Figure~\ref{#1}}}
\def\reffis#1{\mbox{Figures~\ref{#1}}}
%\def\refta#1{\mbox{Tab.~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
%\def\reftas#1{\mbox{Tabs.~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refses#1{\mbox{Sections~\ref{#1}}}
%\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
%\def\refapp#1{\mbox{Appendix~\ref{#1}}}
\def\refapps#1{\mbox{Apps.~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}

%physical units
\newcommand{\eV}{\unskip\,\mathrm{eV}}
\newcommand{\GeV}{\unskip\,\mathrm{GeV}}
\newcommand{\MeV}{\unskip\,\mathrm{MeV}}
\newcommand{\TeV}{\unskip\,\mathrm{TeV}}
\newcommand{\fba}{\unskip\,\mathrm{fb}}
\newcommand{\mba}{\unskip\,\mathrm{mb}}
\newcommand{\pba}{\unskip\,\mathrm{pb}}
\newcommand{\nba}{\unskip\,\mathrm{nb}}


%+X in processes
\newcommand{\X}{X}

%physical particles
\def\mathswitch#1{\relax\ifmmode#1\else$#1$\fi}
\def\mathswitchr#1{\relax\ifmmode{\mathrm{#1}}\else$\mathrm{#1}$\fi}
\def\mathswitchit#1{\relax\ifmmode{#1}\else$#1$\fi}
\newcommand{\PB}{\mathswitchr B}
\newcommand{\PW}{\mathswitchr W}
\newcommand{\PZ}{\mathswitchr Z}
\newcommand{\PAn}{\mathswitchr {A^0}}
\newcommand{\Pg}{\mathswitchr g}
\newcommand{\PH}{\mathswitchr H}
\newcommand{\PHgeneric}{\mathswitchr \phi^0}
\newcommand{\Pe}{\mathswitchr e}
\newcommand{\Pne}{\mathswitch \nu_{\mathrm{e}}}
\newcommand{\Pane}{\mathswitch \bar\nu_{\mathrm{e}}}
\newcommand{\Pnmu}{\mathswitch \nu_\mu}
\newcommand{\Pd}{\mathswitchr d}
%\newcommand{\Pf}{\mathswitchr f}
\newcommand{\Pf}{f}
\newcommand{\Ph}{\mathswitchr h}
\newcommand{\Pj}{\mathswitchr j}
\newcommand{\Pl}{\mathswitch l}
\newcommand{\Plp}{\mathswitch l^+}
\newcommand{\Plm}{\mathswitch l^-}
\newcommand{\Pnl}{\mathswitch {\nu_\Pl}}
\newcommand{\Pnlb}{\mathswitch {\bar{\nu}_\Pl}}
\newcommand{\Pu}{\mathswitchr u}
\newcommand{\Ps}{\mathswitchr s}
%\newcommand{\Pb}{\mathswitchr b}
\newcommand{\Pc}{\mathswitchr c}
\newcommand{\Pb}{\mathswitchr b}
\newcommand{\Pt}{\mathswitchr t}
\newcommand{\Pp}{\mathswitchr p}
\newcommand{\Ppbar}{\overline{\Pp}}
\newcommand{\Pq}{\mathswitchit q}
\newcommand{\Pep}{\mathswitchr {e^+}}
\newcommand{\Pem}{\mathswitchr {e^-}}
\newcommand{\Pepm}{\mathswitchr {e^\pm}}
\newcommand{\Pmum}{\mathswitchr {\mu^-}}
\newcommand{\PWp}{\mathswitchr {W^+}}
\newcommand{\PWm}{\mathswitchr {W^-}}
\newcommand{\PWpm}{\mathswitchr {W^\pm}}
\newcommand{\PWO}{\mathswitchr {W^0}}
\newcommand{\PZO}{\mathswitchr {Z^0}}

\newcommand{\PHu}{\mathswitchr H_\Pu}
\newcommand{\PHd}{\mathswitchr H_\Pd}
\newcommand{\Phn}{\mathswitchr {h^0}}
\newcommand{\PHn}{\mathswitchr {H^0}}

% particle masses
\newcommand{\MB}{\mathswitch {M_\PB}}
\newcommand{\Mf}{\mathswitch {m_\Pf}}
\newcommand{\Ml}{\mathswitch {m_\Pl}}
\newcommand{\Mq}{\mathswitch {m_\Pq}}
\newcommand{\MV}{\mathswitch {M_\PV}}
\newcommand{\MW}{\mathswitch {M_\PW}}
\newcommand{\hMW}{\mathswitch {\hat M_\PW}}
\newcommand{\MWpm}{\mathswitch {M_\PWpm}}
\newcommand{\MWO}{\mathswitch {M_\PWO}}
\newcommand{\MA}{\mathswitch {M_\PAn}}
\newcommand{\MZ}{\mathswitch {M_\PZ}}
\newcommand{\MH}{\mathswitch {M_\PH}}
\newcommand{\Me}{\mathswitch {m_\Pe}}
\newcommand{\Mmy}{\mathswitch {m_\mu}}
\newcommand{\Mta}{\mathswitch {m_\tau}}
\newcommand{\Md}{\mathswitch {m_\Pd}}
\newcommand{\Mu}{\mathswitch {m_\Pu}}
\newcommand{\Ms}{\mathswitch {m_\Ps}}
\newcommand{\Mc}{\mathswitch {m_\Pc}}
\newcommand{\Mb}{\mathswitch {m_\Pb}}
\newcommand{\Mt}{\mathswitch {m_\Pt}}
\newcommand{\GW}{\mathswitch {\Gamma_\PW}}
\newcommand{\GZ}{\mathswitch {\Gamma_\PZ}}

\newcommand{\Mhn}{\mathswitch {M_{\Phn}}}
\newcommand{\MHn}{\mathswitch {M_{\PHn}}}
\newcommand{\MHgeneric}{\mathswitch {M_{\PHgeneric}}}
\newcommand{\Mhntree}{\mathswitch {m_{\Phn}}}
\newcommand{\MHntree}{\mathswitch {m_{\PHn}}}

% complex masses
\newcommand{\muw}{\mathswitch {\mu_{\PW}}}

% shorthands for SM parameters
\newcommand{\scrs}{\scriptscriptstyle}
\newcommand{\sw}{\mathswitch {s_{\scrs\PW}}}
\newcommand{\cw}{\mathswitch {c_{\scrs\PW}}}
%\newcommand{\sw}{\mathswitch {s_\PW}}
%\newcommand{\cw}{\mathswitch {c_\PW}}
%\newcommand{\swbar}{\mathswitch {\bar s_\PW}}
\newcommand{\swbar}{\mathswitch {\bar s_{\scrs\PW}}}
\newcommand{\swfbar}{\mathswitch {\bar s_{\PW,\Pf}}}
\newcommand{\swqbar}{\mathswitch {\bar s_{\PW,\Pq}}}
\newcommand{\Qf}{\mathswitch {Q_\Pf}}
\newcommand{\Ql}{\mathswitch {Q_\Pl}}
\newcommand{\Qq}{\mathswitch {Q_\Pq}}
\newcommand{\vf}{\mathswitch {v_\Pf}}
\newcommand{\af}{\mathswitch {a_\Pf}}
\newcommand{\gesi}{\mathswitch {g_\Pe}^{\sigma}}
\newcommand{\gem}{\mathswitch {g_\Pe}^-}
\newcommand{\gep}{\mathswitch {g_\Pe}^+}
\newcommand{\GF}{\mathswitch {G_\mu}}
\newcommand{\Qu}{\mathswitch {Q_u}}
\newcommand{\HERWIG}{{\tt HERWIG++}}

\newcommand{\vev}{\mathswitch v}
\newcommand{\vevu}{\mathswitch v_\Pu}
\newcommand{\vevd}{\mathswitch v_\Pd}

\newcommand{\sina}{s_\alpha}
\newcommand{\cosa}{c_\alpha}
\newcommand{\sinb}{s_\beta}
\newcommand{\cosb}{c_\beta}
\newcommand{\tana}{t_\alpha}
\newcommand{\tanb}{t_\beta}
\newcommand{\cotb}{\cot \beta}
\newcommand{\alphas}{\alpha_{\mathrm{s}}}
%\newcommand{\ptmiss}{\slashed{{p_{\mathrm{T}}}}}
\newcommand{\ptmiss}{p_{\mathrm{T}}\hspace{-1.0em}/\hspace{0.5em}}
\hyphenation{brems-strah-lung}

%various shorthands
\def\ie{i.e.\ }
\def\eg{e.g.\ }
\def\cf{cf.\ }

% slashed quantities
\newcommand{\as}{a\hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\es}{\varepsilon \hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\ks}{k\hspace{-0.52em}/\hspace{0.1em}}
\newcommand{\ps}{p\hspace{-0.42em}/}%\hspace{0.1em}}
\newcommand{\qs}{q\hspace{-0.5em}/\hspace{0.1em}}
\newcommand{\hb}{h\hspace{-0.5em}\vspace{-0.3em}-\hspace{0.1em}}
\marginparwidth 1.2cm

% orders of magnitude
\newcommand{\ord}{{\cal O}}
\renewcommand{\O}{{\cal O}}
%\newcommand{\C}{{\cal C}}
\newcommand{\Oa}{\mathswitch{{\cal{O}}(\alpha)}}

% various abbreviations
\newcommand{\rE}{{\mathrm{E}}}
\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\re}{{\mathrm{e}}}
\newcommand{\rT}{{\mathrm{T}}}
\newcommand{\rM}{{\mathrm{M}}}
\newcommand{\ieps}{\ri\epsilon}
\newcommand{\rd}{{\mathrm{d}}}
\newcommand{\br}{{\mathrm{br}}}
\newcommand{\soft}{{\mathrm{soft}}}
\newcommand{\onel}{{\mathrm{1-loop}}}
\newcommand{\M}{{\cal {M}}}
\renewcommand{\L}{{\cal L}}
\newcommand{\F}{{\cal {F}}}
\newcommand{\bq}{{\bf q}}
\newcommand{\ehel}{\kappa}
\newcommand{\da}{\Delta\alpha}
\newcommand{\dr}{\Delta\rho}
\newcommand{\dLL}{\Delta_{\mathrm{LL}}}

\newcommand{\cut}{{\mathrm{cut}}}
\newcommand{\llog}{{\mathrm{LL}}}
\newcommand{\FSR}{{\mathrm{FSR}}}
\newcommand{\EW}{{\mathrm{EW}}}
\newcommand{\QCD}{{\mathrm{QCD}}}
\newcommand{\QED}{{\mathrm{QED}}}
\newcommand{\LEP}{{\mathrm{LEP}}}
\newcommand{\OS}{{\mathrm{OS}}}
\newcommand{\SLD}{{\mathrm{SLD}}}
\newcommand{\SM}{{\mathrm{SM}}}
\newcommand{\MSSM}{{\mathrm{MSSM}}}
\newcommand{\SUSY}{{\mathrm{SUSY}}}
\newcommand{\CM}{{\mathrm{CM}}}
\newcommand{\born}{{\mathrm{Born}}}
\newcommand{\virt}{{\mathrm{virt}}}
\newcommand{\coll}{{\mathrm{coll}}}
\newcommand{\sub}{{\mathrm{sub}}}
\newcommand{\ini}{{\mathrm{ini}}}
\newcommand{\fin}{{\mathrm{fin}}}
\newcommand{\fact}{{\mathrm{fact}}}
\newcommand{\nonfact}{{\mathrm{nonfact}}}
\newcommand{\res}{{\mathrm{res}}}
\newcommand{\rec}{{\mathrm{rec}}}
\newcommand{\PA}{{\mathrm{PA}}}
\newcommand{\real}{{\mathrm{real}}}
\newcommand{\veto}{{\mathrm{veto}}}
\newcommand{\LO}{{\mathrm{LO}}}
\newcommand{\NLO}{{\mathrm{NLO}}}
\newcommand{\Int}{{\mathrm{IF}}}
\newcommand{\full}{\mathrm{full}}


% mathematical functions
\def\atn{\mathop{\mathrm{arctan}}\nolimits}
\def\Li{\mathop{\mathrm{Li}_2}\nolimits}
\def\cLi{\mathop{{\cal L}i_2}\nolimits}
\def\Re{\mathop{\mathrm{Re}}\nolimits}
\def\Im{\mathop{\mathrm{Im}}\nolimits}
\def\sgn{\mathop{\mathrm{sgn}}\nolimits}
\def\arc{\mathop{\mathrm{arc}}\nolimits}

% Momenta
\newcommand{\pina}{\mathswitch {p_1}}
\newcommand{\Pina}{\mathswitch {p_1}}
\newcommand{\pinb}{\mathswitch {p_2}}
\newcommand{\Pinb}{\mathswitch {p_2}}
\newcommand{\knu}{\mathswitch {k_{\nu}}}
\newcommand{\Knu}{\mathswitch {k_{\nu}}}
\newcommand{\klb}{\mathswitch {k_{\Pl}}}
\newcommand{\Klb}{\mathswitch {k_{\Pl}}}
\newcommand{\kj}{\mathswitch {p_3}}
\newcommand{\Kj}{\mathswitch {p_3}}
\newcommand{\kga}{\mathswitch {k_{\ga}}}
\newcommand{\Kga}{\mathswitch {k_{\ga}}}
\newcommand{\kw}{\mathswitch {k_{\PW}}}
\newcommand{\Kw}{\mathswitch {k_{\nu}+k_{\Pl}}}

% Helicities
\newcommand{\siga}{\mathswitch {\sigma_1}}
\newcommand{\sigb}{\mathswitch {\sigma_2}}
\newcommand{\taulb}{\mathswitch {\tau_{\Pl}}}
\newcommand{\laj}{\mathswitch {\sigma_3}}
\newcommand{\laga}{\mathswitch {\lambda_{\ga}}}

% Processes
\newcommand{\udnlg}{\mathswitch {\Pu\bar{\Pd}\to\Pl^+\Pnl \mathrm{g}}}
\newcommand{\UDGG} {\mathswitch {\mathrm{gg}\Pd\Pu}}


% modifications for drafts
\newcommand{\mpar}[1]{{\marginpar{\hbadness10000%
                      \sloppy\hfuzz10pt\boldmath\bf#1}}%
                      \typeout{marginpar: #1}\ignorespaces}
\marginparwidth 1.2cm
\marginparsep 0.2cm
\def\draftdate{\relax}
\def\mda{\relax}
\def\mua{\relax}
\def\mla{\relax}
\def\draft{
\def\thtystars{******************************}
\def\sixtystars{\thtystars\thtystars}
\typeout{}
\typeout{\sixtystars**}
\typeout{* Draft mode!
         For final version remove \protect\draft\space in source file *}
\typeout{\sixtystars**}
\typeout{}
\def\draftdate{\today}
\def\mua{\marginpar[\boldmath\hfil$\uparrow$]%
                   {\boldmath$\uparrow$\hfil}%
                    \typeout{marginpar: $\uparrow$}\ignorespaces}
\def\mda{\marginpar[\boldmath\hfil$\downarrow$]%
                   {\boldmath$\downarrow$\hfil}%
                    \typeout{marginpar: $\downarrow$}\ignorespaces}
\def\mla{\marginpar[\boldmath\hfil$\rightarrow$]%
                   {\boldmath$\leftarrow $\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
\def\Mua{\marginpar[\boldmath\hfil$\Uparrow$]%
                   {\boldmath$\Uparrow$\hfil}%
                    \typeout{marginpar: $\Uparrow$}\ignorespaces}
\def\Mda{\marginpar[\boldmath\hfil$\Downarrow$]%
                   {\boldmath$\Downarrow$\hfil}%
                    \typeout{marginpar: $\Downarrow$}\ignorespaces}
\def\Mla{\marginpar[\boldmath\hfil$\Rightarrow$]%
                   {\boldmath$\Leftarrow $\hfil}%
                    \typeout{marginpar: $\Leftrightarrow$}\ignorespaces}
\overfullrule 5pt
\oddsidemargin -15mm
\marginparwidth 29mm
}

% change of eqnarray environment
%  Default is for left-hand side of equations to be flushleft.
%  To make them flushright, \let\@eqnsel = \hfil

\makeatletter
%\let\@eqnsel = \hfil

\def\eqnarray{\stepcounter{equation}\let\@currentlabel=\theequation
\global\@eqnswtrue
\global\@eqcnt\z@\tabskip\@centering\let\\=\@eqncr
%$$\halign to \displaywidth\bgroup\@eqnsel\hskip\@centering
%  $\displaystyle\tabskip\z@{##}$&\global\@eqcnt\@ne
$$\halign to \displaywidth\bgroup\hskip\@centering
  $\displaystyle\tabskip\z@{##}$\@eqnsel&\global\@eqcnt\@ne
  \hskip 2\arraycolsep \hfil${##}$\hfil
  &\global\@eqcnt\tw@ \hskip 2\arraycolsep $\displaystyle\tabskip\z@{##}$\hfil
   \tabskip\@centering&\llap{##}\tabskip\z@\cr}
\def\appendix{\par
 \setcounter{section}{0} \setcounter{subsection}{0}
 \def\thesection{\Alph{section}}}

\newcommand{\gtrless}
{\;\rlap{\raisebox{+.25em}{$>$}}\raisebox{-.25em}{$<$}\;}
\newcommand{\lsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle <}{\sim}$}\;}
\newcommand{\gsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle >}{\sim}$}\;}
\def\asymp#1{\;\raisebox{-.4em}{$\widetilde{\scriptstyle #1}$}\;}
\newcommand{\gl}
{\;\raisebox{.25em}{$>$}\hspace{-.75em}\raisebox{-.2em}{$<$}\;}
\def\dsl{\mathpalette\make@slash}
\def\make@slash#1#2{\setbox\z@\hbox{$#1#2$}%
  \hbox to 0pt{\hss$#1/$\hss\kern-\wd0}\box0}

\newcommand{\mycaption}[2][]{{\begin{center} \parbox{15cm}{{\bf \caption[#1]{\rm {#2}}}} \end{center} }}
%\newcommand{\mycaption}[2][kurz]{{{\bf \caption[#1]{\rm {#2}}}}}

\newcommand{\Vector}[1]{{\left( \begin{array}{c} #1 \end{array} \right) }}
\newcommand{\Matrix}[1]{{\left( \begin{array}{cc} #1 \end{array} \right) }}
\newcommand{\mr}[1]{{\mathrm{#1}}}
\renewcommand{\la}{{\mathcal L}}
\newcommand{\Pbbar}{{\bar{\Pb}}}
\newcommand{\Pdbar}{{\bar{\Pd}}}
\newcommand{\Pubar}{{\bar{\Pu}}}
\newcommand{\Pqbar}{{\bar{\Pq}}}
\newcommand{\MSbar}{{$\overline{\mathrm{MS}}$}}
\newcommand{\DRbar}{{$\overline{\mathrm{DR}}$}}

\newcommand{\comment}[1]{{\noindent {\bf (#1)}}}

\newcommand{\myplot}[9]{
\begin{picture}(0,0)(0,0)
\put(#2,#3){#4}
\begin{rotate}{#8}
\put(#5,#6){#7}
\end{rotate}
\end{picture}
\includegraphics[width=#9]{#1}
}

\newcommand{\RL}{\mathrm{L}}
\newcommand{\RT}{\mathrm{T}}

\makeatother

\def\sub{{\mathrm{sub}}}
\def\sli{{\mathrm{sli}}}
\def\gsub{g^{(\sub)}}
\def\hsub{h}
\def\Gsub{G^{(\sub)}}
\def\Gsli{G^{(\sli)}}
\def\Hsub{H}
\def\cGsub{{\cal G}^{(\sub)}}
\def\cHsub{{\cal H}}
\def\cHsli{{\cal H}}
\def\bcGsub{\bar {\cal G}^{(\sub)}}
\def\bcGsli{\bar {\cal G}^{(\sli)}}
\def\bcHsub{\bar {\cal H}}
\def\ssub{\sigma^{(\sub)}}
\def\gin{g^{\mathrm{(in)}}}
\def\gout{g^{\mathrm{(out)}}}
\def\goutin{g^{\mathrm{(out/in)}}}

\newcommand{\phz}{\phantom{(0)}}

